Loop-Erased Random Walk Branch of Uniform Spanning Tree in Topological Polygons

We consider uniform spanning tree (UST) in topological polygons with $2N$ marked points on the boundary with alternating boundary conditions. In [LPW21], the authors derive the scaling limit of the Peano curve in the UST. They are variants of SLE$_8$. In this article, we derive the scaling limit of the loop-erased random walk branch (LERW) in the UST. They are variants of SLE$_2$. The conclusion is a generalization of [HLW20,Theorem 1.6] where the authors derive the scaling limit of the LERW branch of UST when $N=2$. When $N=2$, the limiting law is SLE$_2(-1,-1; -1, -1)$. However, the limiting law is nolonger in the family of SLE$_2(\rho)$ process as long as $N\ge 3$.

==> tex/discussion.tex <==
\begin{proposition}
The partition function $\PartF$ defined in~\eqref{eqn::partitionfunction} has the following properties. 
\begin{itemize}
\item Second order PDE:
\begin{equation}\label{eqn::PDE}
\left[\partial_y^2+\sum_{j=1}^{2N}\left(\frac{2}{y_j-y}\partial_{y_j}+\frac{1/4}{(y_j-y)^2}\right)\right]\PartF(y; y_1, \ldots, y_{2N})=0.
\end{equation}
\item Conformal covariance: for all Mobius maps $\varphi$ of $\HH$ such that $\varphi(y_1)<\cdots<\varphi(y_{2N})$, 
\begin{equation}\label{eqn::COV}
\PartF(\varphi(y); \varphi(y_1), \ldots, \varphi(y_{2N}))=\varphi'(y)^{-1}\PartF(y; y_1, \ldots, y_{2N}). 
\end{equation}
\end{itemize}
\end{proposition}

From~\eqref{eqn::conformalmap_slitrect}, we see that the partition function defined in~\eqref{eqn::partitionfunction} has the following expression: for $y_1<y<y_2<\cdots<y_{2N}$, 
\begin{equation}\label{eqn::PartF_explicit}
\PartF(y; y_1, \ldots, y_{2N})=\frac{\prod_{\ell=1}^{N-2}(y-\mu^{(\ell)})}{\prod_{j=1}^{2N}(y-y_j)^{1/2}} \left(\int_{y_1}^{y_2} \frac{\prod_{\ell=1}^{N-2}(u-\mu^{(\ell)})\ud u}{\prod_{j=1}^{2N}(u-y_j)^{1/2}} \right)^{-1}. 
\end{equation}


Is it possible to check that $\PartF$ satisfies PDE~\eqref{eqn::PDE} through the express in~\eqref{eqn::PartF_explicit}? If PDE~\eqref{eqn::PDE} holds, then the law of $\varphi(\gamma)$ given $y=\varphi(\LX)$ in Theorem~\ref{thm::lerwconv} is the same as the law of $\SLE_2$ from $y$ to $\infty$ weighted by the following local martingale: 
\[M_t=\prod_{j=1}^{2N}g_t'(y_j)^{-1/8}\times\PartF(W_t; g_t(y_1), \ldots, g_t(y_{2N})).\]

When $N=2$, we have 
\begin{equation}\label{eqn::PartFNequals2}
\PartF(y; y_1, y_2, y_3, y_4)=\prod_{j=1}^4(y-y_j)^{-1/2}\left(\int_{y_1}^{y_2}\frac{\ud u}{\prod_{j=1}^4 (u-y_j)^{1/2}}\right)^{-1}
\end{equation}
Let us simplify the denominator. Setting 
\[w=\left(\frac{u-y_1}{y_{21}}\right)\left(\frac{y_{42}}{y_4-u}\right),\quad q=\frac{y_{21}y_{43}}{y_{31}y_{42}},\] then we have
\begin{align*}
\int_{y_1}^{y_2}\frac{\ud u}{\prod_{j=1}^4 |u-y_j|^{1/2}}=&\frac{1}{\sqrt{y_{31}y_{42}}}\int_0^t\frac{\ud w}{\sqrt{w(1-w)(1-qw)}}=\frac{\pi}{\sqrt{y_{31}y_{42}}}\hF\left(\frac{1}{2}, \frac{1}{2}, 1; q\right). 
\end{align*}
Plugging into~\eqref{eqn::PartFNequals2}, we have 
\[\PartF(y; y_1, y_2, y_3, y_4)=\prod_{j=1}^4|y-y_j|^{-1/2}\times\frac{\pi}{\sqrt{y_{31}y_{42}}}\hF\left(\frac{1}{2}, \frac{1}{2}, 1; q\right).\]

The partition function for $\SLE_2(-1,-1;-1,-1)$ is the following: 
\[\LG(y; y_1, y_2, y_3, y_4)=\prod_{j=1}^4|y-y_j|^{-1/2}\times (y_{21}y_{31}y_{41}y_{32}y_{42}y_{43})^{1/4}.\]

The partition function for $2-\SLE_8$ is the following:
\[\LF(y_1, y_2, y_3, y_4)=cst\times \hF\left(\frac{1}{2}, \frac{1}{2}, 1; q\right)\times\left(\frac{y_{21}y_{41}y_{32}y_{43}}{y_{31}y_{42}}\right)^{1/4}.\]







